ASoBO: Attentive Beamformer Selection for Distant Speaker Diarization in Meetings

Speaker Diarization (SD) aims at grouping speech segments that belong to the same speaker. This task is required in many speech-processing applications, such as rich meeting transcription. In this context, distant microphone arrays usually capture the audio signal. Beamforming, i.e., spatial filtering, is a common practice to process multi-microphone audio data. However, it often requires an explicit localization of the active source to steer the filter. This paper proposes a self-attention-based algorithm to select the output of a bank of fixed spatial filters. This method serves as a feature extractor for joint Voice Activity (VAD) and Overlapped Speech Detection (OSD). The speaker diarization is then inferred from the detected segments. The approach shows convincing distant VAD, OSD, and SD performance, e.g. 14.5% DER on the AISHELL-4 dataset. The analysis of the self-attention weights demonstrates their explainability, as they correlate with the speaker's angular locations.

==> 011_tasks.tex <==
\section{Segmentation Tasks}

\label{sect:tasksssssssssssssss}

This section describes the segmentation tasks considered. 
The labeling procedure for each task is presented in figure~\ref{fig:labels}.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/seg_tasks_labels.pdf}
    \caption{VAD, OSD, and SCD labels along with the reference diarization. VAD and OSD are formulated as a binary frame classification task while SCD is solved as the regression of Gaussian-like functions.}
    \label{fig:labels}
\end{figure}

\vspace{-15pt}

\subsection{Voice Activity and Overlapped Speech Detection}

%Voice Activity detection (VAD) is the task of detecting speech segments from non-speech ones in an audio stream.
VAD is formulated as a framewise binary sequence classification task~\cite{bredin_pyannoteaudio_2020}.
Let $\boldsymbol{X}=[\boldsymbol{X}_0,\dots,\boldsymbol{X}_t,\dots,\boldsymbol{X}_{T-1}]$ be a sequence of features extracted from the audio signal with $T$ being the length of the sequence.
The VAD task aims at predicting the sequence $\boldsymbol{P}=[\boldsymbol{P}_0,\dots,\boldsymbol{P}_t,\dots,\boldsymbol{P}_{T-1}]$, where $\boldsymbol{P}_t = \{p(N_{spk}=0|\boldsymbol{X}_t),p(N_{spk}\geq1|\boldsymbol{X}_t)\}$ is the pseudo-probability of the $t$-th frame to belong to each class.
$N_{spk}$ denotes the number of active speakers in the current frame.

%\subsection{Overlapped Speech Detection}

%Overlapped Speech Detection (OSD) consists in detecting speech segments in which several multiple are simultaneously active.
OSD formulation is similar to VAD.
However, positive labels correspond to frames containing strictly more than one active speaker: $\boldsymbol{P}_t = \{p(N_{spk}\leq1|\boldsymbol{X}_t),p(N_{spk}\geq2|\boldsymbol{X}_t)\}$.

\subsection{Speaker Change Detection}

%Speaker Change Detection (SCD) detects frames in which the currently active speaker is changing.
In this paper, SCD is formulated as a regression task~\cite{hruz2017convolutional}.
This approach consists in estimating functions in which maxima are located at speaker change points.
Speaker changes are represented as Gaussian-like functions\footnote{The variance $\sigma^2$ of the Gaussian functions used as labels is randomized during training. It follows a uniform distribution $\mathcal{U}$ such as $\sigma^2 \sim \mathcal{U}_{[2,7]}$.} following the binary label encoding of~\cite{he_deep_2018}. 
%SCD annotations are illustrated in figure~\ref{fig:labels}.
In this work, the speech-to-non-speech transition is considered as a speaker turn (Fig.~\ref{fig:labels}).


